Weighted Maximum Independent Set of Geometric Objects in Turnstile Streams

We study the Maximum Independent Set problem for geometric objects given in the data stream model. A set of geometric objects is said to be independent if the objects are pairwise disjoint. We consider geometric objects in one and two dimensions, i.e., intervals and disks. Let $\alpha$ be the cardinality of the largest independent set. Our goal is to estimate $\alpha$ in a small amount of space, given that the input is received as a one-pass stream. We also consider a generalization of this problem by assigning weights to each object and estimating $\beta$, the largest value of a weighted independent set. We initialize the study of this problem in the turnstile streaming model (insertions and deletions) and provide the first algorithms for estimating $\alpha$ and $\beta$. For unit-length intervals, we obtain a $(2+\epsilon)$-approximation to $\alpha$ and $\beta$ in poly$(\frac{\log(n)}{\epsilon})$ space. We also show a matching lower bound. Combined with the $3/2$-approximation for insertion-only streams by Cabello and Perez-Lanterno [CP15], our result implies a separation between the insertion-only and turnstile model. For unit-radius disks, we obtain a $\left(\frac{8\sqrt{3}}{\pi}\right)$-approximation to $\alpha$ and $\beta$ in poly$(\log(n), \epsilon^{-1})$ space, which is closely related to the hexagonal circle packing constant. We provide algorithms for estimating $\alpha$ for arbitrary-length intervals under a bounded intersection assumption and study the parameterized space complexity of estimating $\alpha$ and $\beta$, where the parameter is the ratio of maximum to minimum interval length.

==> intro_weighted_int_selection.tex <==
\vspace{-0.1in}
\section{Weighted Interval Selection for Unit Intervals}
\label{sec:turnstile_unit_interval}
In this section, we present an algorithm to approximate the weight $\beta$ of the maximum independent set for unit-length intervals in turnstile streams. Interestingly, we note that estimating $\beta$ has the same complexity as approximating $\alpha$ for unit-length intervals. That is, we obtain a $(2 + \epsilon)$-approximation to $\beta$ in the turnstile model, where the weights are identical. We provide a sketch of this section here and defer details to Appendix \ref{asec:turnstile_unit_interval}.
%We complement this result with a lower bound that shows any $(2-\epsilon)$-approximation to $\alpha$ requires $\Omega(n)$ space. The main algorithmic guarantee we achieve is as follows:
 
\begin{theorem}
\label{thm:weighted_ins_del_unit}
Let $\mathcal{P}$ be a turnstile stream of weighted unit intervals such that the weights are polynomially bounded in $n$ and let $\epsilon \in (0, 1/2)$. There exists an algorithm that outputs an estimator $Y$ such that with probability at least $9/10$ the following guarantees hold:
\begin{enumerate}
    \item $\frac{\beta}{2(1+\epsilon)} \leq Y \leq \beta$.
    \item The total space used is $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$. 
\end{enumerate}
\end{theorem}

We first impose a grid $\Delta$ of side length $1$ and shift it by a random integer. We then snap each interval to the cell containing the center of the interval and partition the real line into odd and even cells. Let $\mathcal{C}_e$ be the set of all even cells and $\mathcal{C}_o$ be the set of all odd cells. By averaging, either $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ or $|\text{\texttt{OPT}}_{\mathcal{C}_o}|$ is at least $\frac{\beta}{2}$. We describe an estimator that gives a $(1+\epsilon)$-approximation to $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ and $|\text{\texttt{OPT}}_{\mathcal{C}_o}|$. W.l.o.g let $|\text{\texttt{OPT}}_{\mathcal{C}_e}| \geq |\text{\texttt{OPT}}_{\mathcal{C}_o}|$.  
%We develop an estimator that gives a $(1+\epsilon)$-approximation to $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ as well as $|\text{\texttt{OPT}}_{\mathcal{C}_o}|$. 
Therefore, taking the max of the two estimators, we obtain a $(2+\epsilon)$-approximation to $\beta$.  


Having reduced the problem to estimating $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$, we observe that each even cell has at most $1$ interval, namely the max weight interval landing in the cell, contributing to $\texttt{OPT}_{\mathcal{C}_e}$. Then, partitioning the cells in $\mathcal{C}_e$ into poly$(\log(n))$ weight classes based on the max weight interval in each cell and approximately counting the number of cells in each weight class suffices to estimate $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ up to a $(1+\epsilon)$-factor. Given such a partition, we can create a substream for each weight class in the partition and compute the $\ell_0$ norm of each substream. However, we do not know the partition of the cells into the weight classes a priori and this partition can vary drastically over the course of stream given that intervals can be deleted. The main technical challenge is to simulate this partition. A key tool we use is to estimate the $\ell_0$ norm of a vector in a turnstile stream, which is a well-studied problem, and we use a result of Kane, Nelson and Woodruff \cite{DBLP:conf/pods/KaneNW10} to obtain a $(1\pm\epsilon)$-approximation in poly$(\frac{\log(n)}{\epsilon})$ space. 

\vspace{-0.1in}
\begin{theorem}{($\ell_0$-Norm Estimation \cite{DBLP:conf/pods/KaneNW10}.)}
\label{thm:ell_0}
In the turnstile model, there is an algorithm for $(1\pm \epsilon)$-approximating the $\ell_0$-norm (number of non-zero coordinates) of a vector using space $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ with success probability $2/3$. 
\end{theorem}
\vspace{-0.05in}

We begin by describing a simple algorithm which obtains a weaker $(9/2+\epsilon)$-approximation to $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ and in turn a $(9+\epsilon)$-approximation to $\beta$. Formally, consider a partition of cells in $\mathcal{C}_e$ into $b = \textrm{poly}(\log(n))$ weight classes $\mathcal{W}_i = \{ c \in \mathcal{C}_e | (1+1/2)^i \leq m(c) < (1+1/2)^{i+1} \}$, where $m(c)$ is the maximum weight of an interval in $c$. Create a substream for each weight class $\mathcal{W}_i$, denoted by $\mathcal{W}'_i$, and feed an input interval into this substream if its weight lies in the range $[(1+1/2)^i, (1+1/2)^{i+1})$. Let $t_i$ be the corresponding $\ell_0$ estimate for substream $\mathcal{W}'_i$. Then, we can approximate the contribution of $\mathcal{W}_i$ by $(1 + 1/2)^{i+1}\cdot t_i$. Summing over the $b$ weight classes gives an estimate for $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$.

Given access to an algorithm for estimating the $\ell_0$-norm, the Na\"ive Approximation Algorithm (\ref{alg:naive_approximation}) satisfies the following guarantee (note, we defer the proof to the appendix): 

\begin{lemma}
\label{lem:NaiveApprox}
The Na\"ive Approximation Algorithm (\ref{alg:naive_approximation}) outputs an estimate $X$ such that with probability $99/100$, $\frac{\beta}{9(1+\epsilon)} \leq X \leq \beta$ and runs in space poly$\left(\frac{\log(n}{\epsilon}\right)$. 
\end{lemma}

\begin{Frame}[\textbf{Algorithm \ref{alg:naive_approximation} : Na\"ive Approximation.}]
\label{alg:naive_approximation}
\textbf{Input:} Given a turnstile stream $\mathcal{P}$ with weighted unit intervals, where the weights are polynomially bounded, $\epsilon$ and $\delta >0$, Na\"ive Approximation outputs a $(9+\epsilon)$-approximation to $\beta$ with probability $1-\delta$.
\begin{enumerate}
	\item Randomly shift a grid $\Delta$ of side length $1$. Partition the cells into even and odd, denoted by $\mathcal{C}_e$ and $\mathcal{C}_o$. 
	\item Consider a partition of cells in $\mathcal{C}_e$ into $b = \textrm{poly}(\log(n))$ weight classes $\mathcal{W}_i = \{ c \in \mathcal{C}_e | (1+1/2)^i \leq m(c) < (1+1/2)^{i+1} \}$, where $m(c)$ is the maximum weight of an interval in $c$ (this is not an algorithmic step since we do not know this partition a priori).
    \item Create a substream for each weight class $\mathcal{W}_i$ denoted by $\mathcal{W}'_i$. 
    \item Feed interval $D(d_j,1, w_j)$ along substream $\mathcal{W}'_i$ if $w_j \in [(1+1/2)^i, (1+1/2)^{i+1})$.
	\item For each substream $\mathcal{W}'_i$, maintain a $(1\pm\epsilon)$-approximate $\ell_0$-estimator (described below). 
	\item Let $t_i$ be the $\ell_0$ estimate corresponding to $\mathcal{W}'_i$. Let $X_e = \frac{2}{9(1+\epsilon)} \sum_{i\in [b]} (1+1/2)^{i+1} t_i$.
    \item Repeat Steps 2-6 for the odd cells $\mathcal{C}_o$ to obtain the corresponding estimator $X_o$. 
\end{enumerate}
\textbf{Output:} max$(X_e, X_o)$
\end{Frame}

We can thus assume we know $\beta$ and $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ up to a constant by initially making $O\left(\log(n)\right)$ guesses and running the Na\"ive Approximation Algorithm for each guess in parallel. At the end of the stream, we know the correct guess up to a constant factor, and thus can output the estimator corresponding to that branch of computation.
A key tool we use in this algorithm is $k$-\texttt{Sparse Recovery}. As mentioned in Berinde et al. \cite{BCIS09}, the $k$-tail guarantee is a sufficient condition for $k$-\texttt{Sparse Recovery}, since in a $k$-sparse vector, the elements of the tail are $0$. We note that the \texttt{Count-Sketch} Algorithm \cite{CCF02} has a $k$-tail guarantee in turnstile streams.

\begin{definition}($k$-\texttt{Sparse Recovery}.)
\label{def:sparse_rec}
Let $x$ be the input vector such that $x$ is updated coordinate-wise in the turnstile streaming model. Then, $x$ is $k$-sparse if $x$ has at most $k$ non-zero entries at the end of the stream of updates. 
Given that $x$ is $k$-sparse, a data structure that exactly recovers $x$ at the end of the stream is referred to as a $k$-\texttt{Sparse Recovery} data structure. 
\end{definition}

Intuitively, we again simulate partitioning cells in $\mathcal{C}_e$ into $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ weight classes according to the maximum weight occurring in each cell. Since we do not know this partition a priori, we initially create $b =O\left(\frac{\log(n)}{\epsilon}\right)$ substreams, one for each weight class and run the $\ell_0$-estimator on each one. We then make $O\left(\frac{\log(n)}{\epsilon}\right)$ guesses for $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ and run the rest of the algorithm for each branch in parallel. Additionally, we run the Na\"ive Approximation Algorithm to compute the right value of $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ up to a constant factor, which runs in space $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$. Then, we create $b = \text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ substreams by agnostically sampling cells with probability $p_i = \Theta\left( \frac{b (1+\epsilon)^i \log(n)}{\epsilon^3 X}\right)$, where $X$ is the right guess for $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$. Sampling at this rate preserves a sufficient number of cells from weight class $\mathcal{W}_i$. We then run a sparse recovery algorithm on the resulting substreams. 

We note that the resulting substreams are sparse. To see this, note we can filter out cells that belong to weight classes $\mathcal{W}_{i'}$ for $i' < i$ by simply checking if the maximum interval seen so far lies in weight classes $\mathcal{W}_{i}$ and higher. Further, sampling with probability proportional to $\Theta\left( \frac{b (1+\epsilon)^i \log(n)}{\epsilon^3 |\text{\texttt{OPT}}_{\mathcal{C}_e}|}\right)$ ensures that the number of cells that survive from weight classes $\mathcal{W}_{i}$ and above are small. Therefore, we recover all such cells using the sparse recovery algorithm. Note, we limit the algorithm to considering weight classes that have a non-trivial contribution to $\text{\texttt{OPT}}_{\mathcal{C}_e}$. 

\begin{Frame}[\textbf{Algorithm \ref{alg:weighted_unit_interval_sampling} : Weighted Unit Interval Turnstile Sampling.}]
\label{alg:weighted_unit_interval_sampling}
\textbf{Input:} Given a turnstile stream $\mathcal{P}$ with weighted (polynomially bounded) unit intervals, $\epsilon$ and $\delta >0$, the sampling procedure outputs a $(2 + \epsilon)$-approximation to $\beta$.
\begin{enumerate}
	\item Randomly shift a grid $\Delta$ of side length $1$. Partition the cells into $\mathcal{C}_e$ and $\mathcal{C}_o$.
    \item For cells in $\mathcal{C}_e$, snap each interval in the input to a cell $c$ that contains its center.
	\item Consider a partitioning of the cells in $\mathcal{C}_e$ into $b = \text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ weight classes $\mathcal{W}_i = \{ c \in \mathcal{C}_e | (1+\epsilon)^i \leq m(c) \leq (1+\epsilon)^{i+1}$ \}, where $m(c)$ is the maximum weight of an interval in $c$ (we do not know this partition a priori.) Create a substream for each weight class $\mathcal{W}_i$ denoted by $\mathcal{W}'_i$. 
    \item Feed interval $D(d_j,1, w_j)$ along substream $\mathcal{W}'_i$ such that $w_j \in [(1+\epsilon)^i, (1+\epsilon)^{i+1})$. Maintain a $(1\pm\epsilon)$-approximate $\ell_0$-estimator for each substream. Let $|\mathcal{W}'_i|$ denote the number of non-empty cells in substream $\mathcal{W}'_i$ and $X_{\mathcal{W}'_i}$ be the corresponding estimate returned by the $\ell_0$-estimator. 
	\item Create $O(\log(n))$ substreams, one for each guess of $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$. Let $X$ be the guess for the current branch of the computation. In parallel, run Algorithm \ref{alg:naive_approximation} which estimates $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ up to a constant factor. Therefore, at the end of the stream, we know a constant factor approximation to the correct value of $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ and use the estimator from the corresponding branch of the computation.    
	\item In parallel, for $i \in [b]$, create substream $\mathcal{S}_i$ by subsampling cells in $\mathcal{C}_e$ with probability $p_i = \Theta\left( \frac{b (1+\epsilon)^i \log(n)}{\epsilon^3 X}\right)$. Note, this sampling is done agnostically at the start of the stream. 
	\item Run a poly$\left(\frac{\log(n)}{\epsilon}\right)$-sparse recovery algorithm on each substream $\mathcal{S}_i$. For substream $\mathcal{S}_i$, filter out cells $c$ such that $m(c) < (1+\epsilon)^i$. Let $\mathcal{S}'_i$ be the set of cells recovered by the sparse recovery algorithm. Let $\mathcal{S}'_{i| \mathcal{W}_i}$ be the cells in $\mathcal{S}'_i$ that belong to weight class $\mathcal{W}_i$. 
	\item Let $X_{\mathcal{W}'} = \sum_{i \in [b]} X_{\mathcal{W}'_i}$. Let $Z_c$ be a random variable such that $Z_c = \frac{(1+\epsilon)^{i+1}}{p_i}$ if $c \in \mathcal{S}'_{i| \mathcal{W}_i}$ and $0$ otherwise. If $X_{\mathcal{W}'_i} \geq \frac{\epsilon X_{\mathcal{W}'} }{(1+\epsilon)^{i+1}b}$, set the estimator for the $i^{th}$ subsample, $Y_i = \sum_{c \in \mathcal{S}'_{i| \mathcal{W}_i}}\frac{X_{\mathcal{W}'_i} Z_c}{\left|\mathcal{S}'_{i| \mathcal{W}_i}\right|}$. 
Otherwise, set $Y_i = 0$. Let $Y_e = \sum_i Y_i$.
    
    %For $c \in \mathcal{S}'_i$ such that $m(c)\leq (1+\epsilon)^{i+1}$, let $Y_i = \sum_{c}\frac{ m(c)}{p_i}$. Else, $Y_i =0$.
    \item Repeat Steps 2-7 for the set $\mathcal{C}_o$ and let $Y_o$ be the corresponding estimator. 
\end{enumerate}
\textbf{Output:} $Y = \textrm{max}(Y_e, Y_o)$.
\end{Frame}



%\begin{proof}
%We observe that for each non-empty cell $c \in \mathcal{C}_e$, there is exactly $1$ interval that can contribute to $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ since each cell of the grid has side length $1$ and all intervals falling in a given cell pairwise intersect. This contributing interval lies in some weight class $\mathcal{W}_i$ and our estimator approximates its weight as $(1+1/2)^{i+1}$. Here, the weights of the intervals are sandwiched between $(1+1/2)^i$ and $(1+1/2)^{i+1}$. Therefore, we overestimate the weight by a factor of at most $3/2$. 

%Further, instead of taking the maximum over each cell $c$, we may have inserted intervals that lie in $c$ into all substreams $\mathcal{W}'_i$. Therefore, we take the sum of our geometrically increasing weight classes over that cell. In the worst case, we approximate the true weight of a contributing interval, $(3/2)^{i+1}$, with $\sum^{i}_{i'=1}(3/2)^{i'+1} = 3((3/2)^{i+1}-1)$. Note, we again overestimate the weight, this time by a factor of $3$. 

%Finally, Theorem \ref{thm:ell_0} overestimates the $\ell_0$-norm of $\mathcal{W}_i$ by at most $1+\epsilon$ with probability at least $2/3$. We boost this probability by running $O(\log(n))$ estimators and taking the median. Union bounding over all $i \in [b]$, we simultaneously overestimate the $\ell_0$-norm of all $\mathcal{W}_i$ by at most $1+\epsilon$ with probability at least $99/100$. Therefore, the overall estimator is a $(9/2+\epsilon)$-approximation to $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$. Rescaling our estimator by the above constant underestimates $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$. Finally, $|\text{\texttt{OPT}}_{\mathcal{C}_e}|\geq \beta/2$ and $\frac{\beta}{(9+\epsilon)} \leq X \leq \beta$. 

%Since our weights are polynomially bounded, we create poly$\left(\log_{1+\epsilon}(n)\right)$ substreams and run a $\ell_0$ estimator from Theorem \ref{thm:ell_0} on each substream. Therefore, the total space used by Algorithm \ref{alg:naive_approximation} is poly$\left(\frac{\log(n}{\epsilon}\right)$.
%\end{proof}


Using the $\ell_0$ norm estimates computed above, we can determine the number of non-empty cells in each of the weight classes. Thus, we create a threshold for weight classes that contribute, such that all the weight classes below the threshold together contribute at most an $\epsilon$-fraction of $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ and we can set their corresponding estimators to $0$. Further, for all the weight classes above the threshold, we can show that sampling at the right rate leads to recovering enough cells to achieve concentration in estimating their contribution. 

Next, we show that the total space used by Algorithm \ref{alg:weighted_unit_interval_sampling} is $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$. We initially create $b =O\left(\frac{\log(n)}{\epsilon}\right)$ substreams, one for each weight class and run an $\ell_0$-estimator on each one. Recall, this requires $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$. We then make $O\left(\frac{\log(n)}{\epsilon}\right)$ guesses for $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ and run the rest of the algorithm for each branch in parallel. Additionally, we run Algorithm \ref{alg:naive_approximation} to compute the right value of $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ up to a constant factor, which runs in space $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$. Then, we create $b$ substreams by sampling cells with probability $p_i = \Theta\left( \frac{b (1+\epsilon)^i \log(n)}{\epsilon^3 X}\right)$, for $i \in [b]$. Subsequently, we run a $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$-sparse recovery algorithm on each one. Note, if each sample is not too large, this can be done in $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ space. Therefore, it remains to show that each sample $\mathcal{S}_i$ is small. 

%The key ingredient in our algorithm is computing the $\ell_1$-heavy hitters in a turnstile stream using the Count-Min Sketch, introduced by Cormode and Muthukrishnan \cite{DBLP:conf/latin/CormodeM04} and obtain the following guarantee:

%\begin{theorem}($\ell_1$ Heavy Hitters.)
%\label{thm:cm_sketch}
%Given $\epsilon, \delta, \phi >0$ and a vector $a$, there exists an algorithm that outputs every item $a_i$ such that $|a_i| \geq (\phi+\epsilon) |a|_1$, and no item $a_i$ such that $|a_i| < \phi |a|_1$ with probability at least $\delta$, and uses space $O\left(\frac{\log(n)}{\epsilon} \log( \frac{2\log(n)}{\delta \phi})\right)$.
%\end{theorem}



%Subsequently, we show that running a $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$-sparse recovery algorithm on each substream recovers the cells that correspond the the weight class $\mathcal{W}_i$ and filters out the cells that belong to other weight classes. 

%We then simulate the partition by subsampling even cells at different sampling rates. Formally, we subsample cells in $\mathcal{C}_e$ $b = \text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ times, with probability proportional to $\Theta( \frac{b (1+\epsilon)^i \log(n)}{\epsilon^3 |\text{\texttt{OPT}}_{\mathcal{C}_e}|})$, for all $i \in [b]$. This presents several issues, as we cannot subsample non-empty cells in turnstile streams a priori.  Further, if a weight class has a small number on non-empty cells, we cannot recover accurate estimates for the contribution of this weight class to $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ at any level of the subsampling. To address the first issue, 

 

%  We do not know this partition a priori, therefore we subsample cells from the input space for a range of probabilities. 
%We then sample a small number of non-empty cells for each weight class and find the heavy hitter cells in each sample set. To sample non-empty cells with a probability $p$ in turnstile streams, we create a substream by sampling every cell in the input space with probability $p$ and running a heavy hitters algorithm on this stream. Note, the empty cells are ignored by the heavy hitters algorithm. We show that an estimator constructed from the heavy hitters suffices.  



\begin{lemma}
\label{lem:weighted_ins_del_unit_space}
Given a turnstile stream $\mathcal{P}$, with probability at least $99/100$, the Weighted Unit Interval Turnstile Sampling procedure (Algorithm \ref{alg:weighted_unit_interval_sampling}) samples $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ cells from the grid $\Delta$.  
\end{lemma}
\vspace{-0.2in}
\begin{proof}
For $i \in [b]$, let $\mathcal{S}_i$ be a substream of cells in $\mathcal{C}_e$, sampled with probability $p_i$ and having an interval with weight at least $(1+\epsilon)^i$ since we filter out all cells with smaller weight. Then, by an averaging argument, the total number of cells with an interval of weight at least $(1+\epsilon)^{i}$ is at most $\frac{\beta}{(1+\epsilon)^i}$. Sampling with probability $p_i = \Theta\left( \frac{b (1+\epsilon)^i \log(n)}{\epsilon^3 X}\right)$, the expected number of cells from $\mathcal{W}_i$ that survive in $\mathcal{S}_i$ is at most $p_i \frac{\beta}{(1+\epsilon)^i} = \text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ in expectation. Next, we show that they are never much larger than their expectation. Let $X_c$ be the indicator random variable for cell $c \in \mathcal{W}_i$ to be sampled in $\mathcal{S}_i$ and let $\mu$ be the expected number of cells in $\mathcal{S}_i$. By Chernoff bounds, $\Pr\left[\sum_c X_c \geq (1+\epsilon)\mu\right] \leq \textrm{exp}\left(-\frac{2\epsilon^2 \textrm{poly}(\log(n))}{\textrm{poly}(\epsilon)}\right) \leq 1/n^k$
for some large constant $k$. A similar argument holds for the number of cells from weight class $\mathcal{W}_{i'}$, for $i' > i$, surviving in substream $\mathcal{S}_i$. Note, for all $i' < i$, we never include such a cell from weight class $\mathcal{W}_{i'}$ in our sample $\mathcal{S}_i$, since the filtering step rejects all cells that do not contain an interval of weight at least $(1+\epsilon)^i$. Union bounding over the events that cells $c \in \mathcal{W}_{i'}$ get sampled in $\mathcal{S}_{i}$, for $i'\geq i$, the cardinality of $\mathcal{S}_i$ is at most $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ with probability at least $1-1/n^{k'}$ for an appropriate constant $k'$. Since we create $b$ such substreams for $\mathcal{C}_e$, we can union bound over such events in each of them and thus $\bigcup_{i\in [b]} |\mathcal{S}_i|$ is at most $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ with probability at least $99/100$. Since $|\mathcal{C}_e|$ is $|\Delta|/2$, the same result holds for the total cells sampled from $\Delta$. Therefore, the overall space used by Algorithm \ref{alg:weighted_unit_interval_sampling} is $\text{poly}\left(\frac{\log(n)}{\epsilon}\right)$.  
\end{proof}


Next, we show that the estimate returned by our sampling procedure is indeed a $(2 + \epsilon)$-approximation. We observe that the union of the $\mathcal{W}_i$'s form a partition of $\mathcal{C}_e$. Therefore, it suffices to show that we obtain a $(1+\epsilon)$-approximation to the \texttt{WIS} for each $\mathcal{W}_i$ with good probability. Let $c$ denote a cell in $\mathcal{W}_i$ and $\text{\texttt{OPT}}_c$ denote the \texttt{WIS} in cell $c$. We create a substream for each weight class $\mathcal{W}_i$ denoted by $\mathcal{W}'_i$ and let $X_{\mathcal{W}'_i}$ be the corresponding estimate returned by the $\ell_0$ norm of $\mathcal{W}'_i$. Let $X_{\mathcal{W}'} = \sum_{i \in [b]} X_{\mathcal{W}'_i}$ denote the sum of the estimates across the $b$ substreams. We say that weight class $\mathcal{W}_i$ contributes if $X_{\mathcal{W}'_i} \geq \frac{\epsilon X_{\mathcal{W}'} }{(1+\epsilon)^{i+1}b}$. 
Note, if we discard all the weight classes that do not contribute we lose at most an $\epsilon$-fraction of $\beta$ (as shown below). Therefore, setting the estimators corresponding to classes that do not contribute to $0$ suffices. The main technical hurdle remaining is to show that if a weight class contributes we can accurately estimate $|\texttt{OPT}_{\mathcal{W}_i}|$.   

\vspace{-0.08in}
\begin{lemma}
\label{lem:weighted_ins_del_unit_approx}
Let $Y_e = \sum_i Y_i$ be the estimator returned by Algorithm \ref{alg:weighted_unit_interval_sampling} for the set $\mathcal{C}_e$. Then, $Y_e =(1\pm\epsilon)|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ with probability at least $99/100$.
\end{lemma}
\vspace{-0.15in}
\begin{proof}
We defer the details of this proof to Appendix \ref{asec:turnstile_unit_interval}.
\begin{comment}
We first consider the case when $\mathcal{W}_i$ contributes, i.e., $X_{\mathcal{W}'_i} \geq \frac{\epsilon X_{\mathcal{W}'} }{(1+\epsilon)^{i+1}b}$. Note, $X_{\mathcal{W}'} = \sum_{i \in [b]} X_{\mathcal{W}'_i}$ is a $(1\pm \epsilon)$-approximation to the number of non-empty cells in $\mathcal{W}$ with probability at least $1 - n^{-k}$, where $\mathcal{W} = \bigcup_{i \in [b]} \mathcal{W}_i$, since the $\ell_0$-estimator is a $(1\pm \epsilon)$-approximation to the number of non-empty cells in $\mathcal{W}_i$ simultaneously for all $i$ with high probability and the $\mathcal{W}_i$'s are disjoint. Recall, $X$ is the correct guess for $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$. Therefore, $
(1+\epsilon)^i X_{\mathcal{W}'_i} = \Omega\left( \frac{\epsilon  X}{(1+\epsilon)b}\right) = \Omega\left(\frac{\epsilon X}{(1+\epsilon)b}\right)$.
Then, sampling at a rate $p_i = \Theta( \frac{b (1+\epsilon)^i \log(n)}{\epsilon^3 X})$ implies at least $\Omega\left(\frac{\epsilon X}{(1+\epsilon)^{i+1} b}\right)\cdot\Theta( \frac{b (1+\epsilon)^i \log(n)}{\epsilon^3 X})  = \Omega\left(\frac{\log(n)}{(1+\epsilon)\epsilon^2}\right)$ cells from $\mathcal{W}_i$ survive in expectation. Let $X_c$ denote an indicator random variable for cell $c \in \mathcal{W}_i$ being in substream $\mathcal{S}_i$. Then, by a Chernoff bound, $\Pr\left[ \sum_{c\in \mathcal{W}_i} X_c  \leq (1-\epsilon)\left(\frac{\log(n^{-c})}{2\epsilon^2}\right)\right] \leq \textrm{exp}\left(\frac{-2\epsilon^2 \log(n^{-c})}{2\epsilon^2}\right) \leq n^{-c}$
for some constant $c$. Union bounding over all the random events similar to the one above for $i\in [b]$, simultaneously for all $i$, the number of cells from $\mathcal{W}_i$ in $\mathcal{S}_i$ is at least $\Omega\left(\frac{\log(n)}{\epsilon^2}\right)$ with probability at least $1-1/n^k$ for some constant $k$. Note, for $i'< i$, no cell $c \in \mathcal{W}_{i'}$ exists in $\mathcal{S}_i$ since the filter step removes all cells $c$ such that $m(c) < (1+\epsilon)^i$.  

Next, consider a weight class $\mathcal{W}_{i'}$ for $i' > i$ such that it contributes. We upper bound the number of cells from $\mathcal{W}_{i'}$ that survive in substream $\mathcal{S}_i$. Note, weight class $\mathcal{W}_{i'}$ contains at most $\frac{\beta}{(1+\epsilon)^{i+1}}$ non empty cells for $i'>i$. In expectation, at most $\frac{\beta}{(1+\epsilon)^{i+1}}\cdot p_i =  O\left(b\frac{\log(n)}{(1+\epsilon)\epsilon^3}\right)$ cells from $\mathcal{W}_{i'}$ survive in sample $\mathcal{S}_i$, for $i'>i$. By a Chernoff bound, similar to the one above, simultaneously for all $i'>i$, at most $O\left(b\frac{\log(n)}{(1+\epsilon)\epsilon^3}\right)$ cells from $\mathcal{W}_{i'}$ survive, with probability at least $1-1/n^{k'}$.
%Further, in expectation, the fraction of $|\text{\texttt{OPT}}_{\mathcal{C}_e}|$ in the union of our samples $\mathcal{S}_i$ is $p_i |\text{\texttt{OPT}}_{\mathcal{C}_e}| = \Theta(\frac{(1+\epsilon)^i b \log(n)}{\epsilon^3})$. 

Now, we observe that the total number of cells that survive the sampling process in substream $\mathcal{S}_i$ is $\text{poly}\left(\log(n), \epsilon^{-1}\right)$ and therefore, they can be recovered exactly by the $\text{poly}\left(\log(n), \epsilon^{-1}\right)$-sparse recovery algorithm. Let the resulting set be denoted by $\mathcal{S}'_i$. We can also compute the number of cells that belong to weight class $\mathcal{W}_i$ that are recovered in the set $\mathcal{S}'_i$ and we denote this by $|\mathcal{S}'_{i | \mathcal{W}_i}|$. Recall, the corresponding estimator is $Y_i = \sum_{c \in \mathcal{S}'_{i| \mathcal{W}_i}}X_{\mathcal{W}'_i} Z_c/|\mathcal{S}'_{i| \mathcal{W}_i}|$, where $Z_c = \frac{(1+\epsilon)^{i+1}}{p_i}$ if $c \in \mathcal{S}'_{i| \mathcal{W}_i}$ and $0$ otherwise. We first show we obtain a good estimator for $|\texttt{OPT}_{\mathcal{W}_i}|$ in expectation: $\E\left[ Y_i \right]  = \E \left[ \sum_{c \in \mathcal{S}'_{i| \mathcal{W}_i}}\frac{X_{\mathcal{W}'_i} Z_c}{\left|\mathcal{S}'_{i| \mathcal{W}_i}\right|} \right] = (1+\epsilon)^{i+1} X_{\mathcal{W}'_i} 
= (1\pm \epsilon) (1+\epsilon)^{i+1} |\mathcal{W}'_i| 
= (1\pm \epsilon)(1+\epsilon) |\text{\texttt{OPT}}_{\mathcal{W}_i}|  = (1\pm 4\epsilon) |\text{\texttt{OPT}}_{\mathcal{W}_i}|
$.
%for $i' \geq i $, we observe that any cell $c \in \mathcal{W}_{i'}$ which survives the sampling process has weight at least $(1+\epsilon)^i$, and therefore it is an $\ell_1$-heavy hitter with parameter $\phi_i$. By Theorem \ref{thm:cm_sketch}, we can recover all such cells $c$ with high probability. Additionally, for $i' < i$, we get no cell $c \in \mathcal{W}_{i'}$ since they cannot be heavy hitters and are removed from the sample. 
%Recall, $\Omega(\frac{\log(n)}{\epsilon^2})$ cells from $\mathcal{W}_i$ are sampled in $\mathcal{S}_i$, which is sufficient to show the concentration of $Y_i$ around $|\texttt{OPT}_{\mathcal{W}_i}|$. For $c \in \mathcal{W}_i$, let $Y^c_i$ be a random variable that is $m(c)/p_i$ if $c \in \mathcal{S}_i$ and $0$ otherwise and let $Y_i = \sum_{c\in \mathcal{S}_i} Y^c_i = \sum_{c \in \mathcal{W}_i} Y^c_i$. Observe, 
%\begin{equation*}
%\begin{split}
%\E\left[ Y_i \right] & = \E \left[ \sum_{c \in \mathcal{S}'_{i| \mathcal{W}_i}}\frac{X_{\mathcal{W}'_i} Z_c}{\left|\mathcal{S}'_{i| \mathcal{W}_i}\right|} \right] = (1+\epsilon)^{i+1} X_{\mathcal{W}'_i} 
%= (1\pm \epsilon) (1+\epsilon)^{i+1} |\mathcal{W}'_i| \\
%&= (1\pm \epsilon)(1+\epsilon) |\text{\texttt{OPT}}_{\mathcal{W}_i}|  = (1\pm 4\epsilon) |\text{\texttt{OPT}}_{\mathcal{W}_i}|
%\end{split}
%\end{equation*}
Since we know that $|\mathcal{S}'_{i | \mathcal{W}_i}| = $ $\Omega(\frac{\log(n)}{(1+\epsilon)\epsilon^2})$, we show that our estimator concentrates. Note, $\E\left[ Y_i \right] = (1+\epsilon)^{i+1} X_{\mathcal{W}'_i} = \Omega(\frac{\epsilon X}{\log(n)})$. Further, $0 \leq Z_c \leq \frac{(1+\epsilon)^{i+1}}{p_i} = O\left( \frac{(1+\epsilon)^{i+1} \epsilon^3 X}{b (1+\epsilon)^i \log(n)} \right)$. Therefore, $ \mathlarger{\sum_{c \in \mathcal{S}'_{i| \mathcal{W}_i}}} \left(\frac{X_{\mathcal{W}'_i} Z_c}{\left|\mathcal{S}'_{i| \mathcal{W}_i}\right|} \right)^2 = O\left( \left(\frac{(1+\epsilon)^{i+1} \epsilon^3 X \cdot X_{\mathcal{W'}_i}}{b (1+\epsilon)^i \log(n)}\right)^2 \frac{1}{\left|\mathcal{S}'_{i| \mathcal{W}_i}\right|} \right)$ and $X_{\mathcal{W}'_i} = \text{poly}\left(\frac{\log(n)}{\epsilon}\right)$ 
By a Hoeffding bound, $\Pr[ |Y_i - E\left[Y_i\right]|  \geq \epsilon E\left[ Y_i \right]]  \leq 2 \textrm{exp}\left(-2\epsilon^2 E\left[ Y_i \right]^2/\sum_{c \in \mathcal{S}'_{i| \mathcal{W}_i}} \left(X_{\mathcal{W}'_i} Z_c/|\mathcal{S}'_{i| \mathcal{W}_i}| \right)^2 \right )$
% \leq 2 \textrm{exp}\left(\frac{\Omega(\log(n))}{1+\epsilon}\right) \leq 1/n^k
%\begin{equation*}
%\begin{split}
%\Pr\Big[ |Y_i - E\left[Y_i\right]|  \geq \epsilon E\left[ Y_i \right]\Big] & \leq 2 \textrm{exp}\left(\frac{-2\epsilon^2 E\left[ Y_i \right]^2}{\mathlarger{\sum_{c \in \mathcal{S}'_{i| \mathcal{W}_i}}} \left(\frac{X_{\mathcal{W}'_i} Z_c}{\left|\mathcal{S}'_{i| \mathcal{W}_i}\right|} \right)^2 }\right ) 
% \leq 2 \textrm{exp}\left(\frac{\Omega(\log(n))}{1+\epsilon}\right) \leq 1/n^k
%\end{split}
%\end{equation*}
for some constant $k$. Therefore, union bounding over all $i$, $Y_i$ is a $(1 \pm \epsilon)^2$-approximation to $|\text{\texttt{OPT}}_{\mathcal{W}_i}|$ with probability at least $1 - 1/n$. Therefore, if $\mathcal{W}_i$ contributes we obtain a $(1 \pm \epsilon)$-approximation to $|\text{\texttt{OPT}}_{\mathcal{W}_i}|$.   
In the case where $\mathcal{W}_i$ does not contribute, we set the corresponding estimator to $0$. Note, $X_{\mathcal{W}'_i} < \frac{\epsilon X_{\mathcal{W}'} }{(1+\epsilon)^{i+1}b} = \frac{\epsilon (1\pm \epsilon) |\texttt{OPT}_{\mathcal{W}}|}{b} = O(\frac{\epsilon \beta}{b})$. Note, since there are at most $b$ weight classes, discarding all weight classes that do not contribute discards at most $O(\epsilon \beta)$. We therefore lose at most an $\epsilon$-fraction of $\beta$ by setting the $Y_i$ corresponding to non-contributing weight classes to $0$. 

%by a Chernoff bound, the number of samples we get is smaller than $O\left( \frac{\epsilon W}{b(1+\epsilon)^i}\right) $ with high probability. Therefore, our estimate $Y_i < \Theta\left(\frac{\log(n)}{\epsilon^3}\right)$ and can be set to $0$. Note, in this case we do not obtain a concentration, but we also do not overcount. The proof of Theorem \ref{thm:weighted_ins_del_unit} immediately follows from union bounding the two cases above and Lemma \ref{lem:weighted_ins_del_unit_space}.
\end{comment}
\end{proof}
Combining Lemmas \ref{lem:NaiveApprox} and  \ref{lem:weighted_ins_del_unit_approx} finishes the proof for Theorem \ref{thm:weighted_ins_del_unit}. 

==> massive_lowerbound.tex <==
\section{Arbitrary Length Intervals in Turnstile Streams} 
We now focus on estimating $\alpha$ for arbitrary-length intervals. We first 
rule out any constant factor approximation to $\alpha$ in 
poly$\left(\frac{\log(n)}{\epsilon}\right)$ space. Note, this also holds for estimating $\beta$. %To find the source of complexity, we study the problem under additional assumptions and parametrization. 
To cope with this hardness, we isolate two sources of hardness - the maximum 
degree of the interval intersection graph, and the maximum length of an 
interval. 
The problem turns out to be tractable under a bounded degree assumption, i.e., we show an algorithm that achieves a $(1+\epsilon)$-approximation to $\alpha$
given that the maximum degree is upper bounded by poly$\left(\frac{\log(n)}
{\epsilon}\right)$. We also parameterize the problem with respect to the 
maximum length of an interval, $W_{max}$ (assuming the minimum length is $1$), and give an algorithm using poly$\left(W_{max} \frac{\log(n)}
{\epsilon}\right)$ space.     


\subsection{Lower bound for Arbitrary Length Intervals}
Here, we define a new communication problem and give information complexity arguments 
%developed in Bar-Yossef et. al. \cite{BJKS02} 
to lower bound its communication complexity. 
The main theorem we prove is the following:

\begin{theorem}
\label{thm:lowerbound_arb_len_unit_wt_ins_del}
Let $\mathcal{P}$ be a turnstile stream of arbitrary-length intervals such 
that the lengths are polynomially bounded in $n$. Any $O(c)$-approximate 
algorithm for $\alpha$ requires $\Omega\left(n^{\frac{1}{c}}\right)$ space. 
\end{theorem}

We begin by defining the communication complexity problem and reducing it to
the unit-weight arbitrary-length interval selection problem. We work in the 
simultaneous multi-party randomized communication complexity model, where 
there are $t$ players, $P_1, P_2, \ldots, P_t$, with private randomness as 
well as a common publicly shared random string $R$, and the objective is to 
communicate with a central referee who computes a function $f: X_1 \times X_2 
\ldots \times X_t \to \{0, 1\} $ on the joint inputs of the players. The 
communication is one-way and each player is allowed to send exactly one 
message to the referee. Given $x_i$ as an input to player $i$, let 
$\Pi\left(x_1, x_2, \ldots x_t\right)$ be the random variable that denotes the 
transcript between the players and the referee when they execute a protocol 
$\Pi$. For $i \in [t]$, let $\Pi_i$ denote the message sent by $P_i$ to the 
referee. 
A protocol $\Pi$ is called a $\delta$-error protocol for function $f$ if there 
exists a function $\Pi_{out}$ such that for every input 
$Pr\left[\Pi_{out}\left(\Pi(x_1, x_2, \ldots x_n)\right) = f(x_1, x_2, \ldots 
x_n)\right] \geq 1 - \delta$. The communication cost of a protocol, denoted by 
$|\Pi|$, is the maximum length of $\Pi\left(x_1, x_2, \ldots, x_n\right)$ over 
all possible inputs and random coin flips of all the $t$ players and the 
referee. The randomized communication complexity of a function $f$, 
$R_{\delta}(f)$, is the communication cost of the best $\delta$-error protocol 
for computing $f$.


\begin{definition}(\textsf{Index Partition}.)
Let $Y$ denote a $s \times t$ matrix such that each column of $Y$ is the 
column vector $[1, ,2 , \ldots , s]$. Let $\pi(Y)$ be a $s \times t$ matrix 
formed by applying a permutation to each column of $Y$. 
We define an \textit{Index Partition} $\mathcal{S} = \{\mathcal{S}_1, \mathcal{S}_2, \ldots, \mathcal{S}_s\}$ where $\mathcal{S}_i$ is the $i^{th}$ 
row of $\pi(Y)$. 
\end{definition}


\begin{definition}(\textsf{Path}.)
Let $X$ be a binary $s \times t$ matrix and let $\mathcal{S}$ be a 
\textit{Index Partition} as defined above. Then, we define a path to be a 
length $t$ row vector $\mathcal{S}_j \in \mathcal{S}$ such that each entry in 
$\mathcal{S}_j$ is an index in the range $[s]$. We can evaluate matrix $X$ 
along the path $\mathcal{S}_j$ by looking at the entry in the $i^{th}$ column 
of $X$ indexed by $\mathcal{S}_j(i)$, for $i \in [t]$. We denote this by 
$X_{\mathcal{S}_j}$.
\end{definition}


\begin{definition}(\textsf{Simultaneous Multi-Party Augmented Path Disjointness}, \texttt{APD$_{s,t}$}.) \\
Let $\mathcal{S} = \{\mathcal{S}_1, \mathcal{S}_2, \ldots, \mathcal{S}_s\}$ be a  \textit{Index Partition} as defined above.  
Let $j^*$ be a special index that determines a path $\mathcal{S}_{j^*} = \left( \mathcal{S}_{j^*}(1),\mathcal{S}_{j^*}(2), \ldots \mathcal{S}_{j^*}(t)  \right)$ in the Index Partition $\mathcal{S}$. Let $P_1, P_2, \ldots P_{t}$ 
be $t$ players with access to public randomness. Then, player $P_i$ receives 
as input $X^i_\mathcal{S} = \left(X^i_{\mathcal{S}_1(i)}, 
X^i_{\mathcal{S}_2(i)}, \ldots,  X^i_{\mathcal{S}_s(i)} \right)$ as well as an 
integer, $\ell_i =\sum^{i-1}_{k=1} \frac{\mathcal{S}_{j^*}(k)W}{s^{kt}}$, that 
denotes a normalized sum of the indices along path $\mathcal{S}_{j^*}$ for all 
the previous players.  
The referee receives as input the path $\mathcal{S}_{j^*}$. The referee also 
gets the bit vectors of the players along the all the paths that are 
lexicographically less than $\mathcal{S}_{j^*}$, namely $\{ X_{\mathcal{S}_{1}}, X_{\mathcal{S}_{2}} \ldots X_{\mathcal{S}_{j^* -1}} \}$. 
Let this set be denoted by $X_{\mathcal{S}_{<j^*}}$. 
Further, we are promised that each path $\mathcal{S}_{j}$ corresponds to a bit 
vector $X_{\mathcal{S}_j}$ such that it either has $t$ $1$s or at most one 
$1$. The referee outputs the disjointness function along path 
$\mathcal{S}_{j^*}$ i.e. outputs $1$ iff $\wedge_{i \in [t]}  
X^{i}_{\mathcal{S}_{j^*}(i)} = 1$.   
\end{definition}

Intuitively, in the above communication problem, each player gets a length $s$ 
bit-vector that is a permutation of a column of $X$, while being oblivious to 
the underlying permutation. 
Each player also gets as input a number, $\ell_i = \sum^{i-1}_{k=1} 
\frac{\mathcal{S}_{j^*}(k)W}{s^{kt}}$, that denotes a normalized sum of 
previous players indices along the path $\mathcal{S}_{j^*}$. Since the 
underlying permutation was chosen uniformly at random, the integer provides no 
information to the player about the index that corresponds to path 
$\mathcal{S}_{j^*}$. 

Note, without the random permutations and the integer $\ell_i$, the above 
problem is simply set disjointness, with augmented information, where the 
referee is interested in computing the disjointness function for $j^*$-{th} 
index of each player's input and additionally has access to each players input 
for indices $j < j^*$. In the matrix notation, this corresponds to computing 
$\wedge_{i \in [t]} X^i_{j^*}$, given $X_{< j^*}$ and $j^*$.

At first glance the additional integer $\ell_i$ might seem superfluous but it 
is critical to our reduction. Note, it is important that $\ell_i$ is 
uncorrelated with the special index for player $i$. Observe, if each player 
also receives $j^*$ as input, they can just send their $j^*$-th bit to the 
referee, making the communication problem easy. By introducing the random 
permutations, $ell_i$ appears to be a random integer uncorrelated with the 
input or the special index for the $i$-th player. The referee now computes 
disjointness along a path in the matrix indexed by $j^*$. The $i$-th player 
knows $\ell_i = \sum^{i-1}_{k=1} \frac{\mathcal{S}_{j^*}(k)W}{s^{kt}}$ but 
gains no information about $S_{j^*}(i)$ as they are independent. 

We begin with a reduction that any algorithm achieving a $c$-approximation to 
$\alpha$ for arbitrary length intervals solves the Simultaneous Multi-Party 
Augmented Path Disjointness, \texttt{APD$_{s,t}$}. A key observation in our 
lower bound is that linear sketches achieve optimal space bounds in strict 
turnstile streams, which was shown by Ai et. al. \cite{AHLW16}. Here
a strict turnstile stream means that an interval can be deleted, but not unless it had previously
been inserted (to contrast it with the general turnstile model, where one could have negative
intervals, which are unnatural in our context). 

\begin{theorem}(\text{Theorem 4.1}, \cite{AHLW16})
\label{thm:sketch_strict_turnstile}
Suppose a randomized algorithm $\mathcal{A}$ solves a problem $\mathcal{P}$ in 
the strict turnstile model with probability at least $1-\delta$. Then there 
exists an algorithm $\mathcal{B}$ implemented by maintaining a linear sketch 
$A\cdot x $ mod $q$ in the stream, where $A$ is a random $r\times n$ integer 
matrix and $q$ is a positive integer of length $r$ such that $\mathcal{B}$ 
solves $\mathcal{P}$ in the strict turnstile model with probability at least 
$1 - 6\delta$ and the space used by any deterministic instance of 
$\mathcal{B}$ is no more than the space used by $\mathcal{A}$.
\end{theorem}

Therefore, by Theorem \ref{thm:sketch_strict_turnstile} a streaming algorithm \texttt{Alg} can be simulated as a linear sketch computed by each player on 
their respective input independently. Each player then communicates the sketch 
to the referee, and by linearity, the referee can combine the sketches to 
compute $f$ on the joint input. Note that the referee knows the sketching 
matrix using the public coin. This enables us to have a valid protocol in the 
simultaneous multi-party communication model using \texttt{Alg} as a 
subroutine. We now show the reduction from \texttt{APD$_{s,t}$} to an 
algorithm that approximates $\alpha$ for arbitrary length intervals in the 
one-pass turnstile model. 



\begin{lemma}(\textsf{Streaming Reduction.})
\label{lem:streamingreduction}
Let \texttt{Alg} be a one-pass turnstile streaming algorithm that, with 
constant probability, obtains a $(t/2)$-approximation to $\alpha$ for 
arbitrary length intervals and uses $m$ bits of space. Then, there exists a 
valid protocol $\Pi$ for \texttt{APD$_{s,t}$} that uses \texttt{Alg} as a 
subroutine such that the total communication is proportion to $m$. 
\end{lemma}
\begin{proof}
Let $W$ denote the max length of an interval in the stream. We set $W$ to a 
large polynomial in $n$. Given an instance of \texttt{APD$_{s,t}$}, recall the 
first player gets $X^1_{\mathcal{S}}$. She then creates a turnstile stream as 
follows : for $j \in [s]$, if $X^1_{\mathcal{S}}(j) = 1$, insert an interval 
with the left endpoint at $0$ and the right end point at $\frac{j W}{s^{t}}$. 
We note that all inserted intervals are open at both endpoints. If 
$X^1_{\mathcal{S}}(j) = 0$, she does not insert any interval into her stream. 
She then creates a linear sketch of her input, denoted by $\mathcal{B}_1$ and 
communicates it to the referee. 

Each subsequent player $P_i$ gets the vector $X^i_{\mathcal{S}}$ along with 
the sum of the indices along path $\mathcal{S}_{j^*}$ for all the previous 
players, denoted by $\ell_i = \sum^{i-1}_{k=1} \frac{\mathcal{S}_{j^*}(k)W}
{s^{kt}}$. Player $P_i$ independently creates a stream as follows: they select 
their left endpoint to be $\ell_i$. If $X^i_{\mathcal{S}}(j) = 1$, the 
rightmost endpoint of the interval streamed by $P_i$ is $\ell_i +  \frac{jW}{s^{it}}$. 
Recall, $\ell_i$ is given as input to the $i^{th}$ player and is crucial for 
them to decide the left end point of each inserted interval. The player $P_i$ 
then creates a linear sketch of their input and sends $\mathcal{B}_i$ to the 
referee. We note that the length of the intervals are exponential in $t$, but 
this suffices since we eventually we set $s=n/t$ and $t$ to be a constant. 

Recall the referee gets as input a path $\mathcal{S}_{j^*}$, and the bit 
vectors of the players along the all the paths that are lexicographically less 
than $\mathcal{S}_{j^*}$, namely $\{ X_{\mathcal{S}_{1}}, X_{\mathcal{S}_{2}} 
\ldots X_{\mathcal{S}_{j^* -1}} \}$, denoted by $X_{\mathcal{S}_{< j^*}}$. The 
referee then combines the linear sketches received from each player. The 
referee proceeds to delete all intervals which correspond to non-zero elements 
in $X_{ \mathcal{S}_{< j^*}}$. Note, this corresponds to deleting all 
intervals inserted in paths lexicographically less than $\mathcal{S}_{j^*}$. 
The referee can indeed execute this as $\mathcal{S}_{j^*}$ determines the left 
endpoints of the inserted intervals and the non-zero bits in 
$X_{\mathcal{S}_{< j^*}}$ (combined with their corresponding index) determine 
the length of each interval. Finally, the referee queries the combined sketch 
to obtain an estimate $Y$ for $\alpha$. If $Y < t$, the referee outputs $0$, 
else the referee outputs $1$. It is left to argue that if 
$X_{\mathcal{S}_{j^*}}$ has at most one $1$, $\alpha \leq 2$ and if 
$X_{\mathcal{S}_{j^*}}$ has all $1$s, $\alpha = t$. Assuming this is true, any $(t/2)$-approximation algorithm suffices to solve \texttt{APD$_{s,t}$}. 

Consider the case where Player $P_i$ actually inserts an interval, 
corresponding to the $j^{th}$ bit of their input. The left end point of any 
such interval is $\sum^{i-1}_{k=1} \frac{\mathcal{S}_{j^*}(k)W}{s^{kt}}$ and 
the length of the interval is $\frac{j W}{s^{it}}$. Note, left end point of 
any interval inserted by the last player is $\sum^{t-1}_{k=1} \frac{\mathcal{S}_{j^*}(k)W}{s^{kt}}$. Further, this is also the rightmost 
left end point of any interval in the set. The distance between the left end 
point of players $P_i$ and $P_t$ is 
\begin{equation*}
\begin{split}
\sum^{t-1}_{k=i} \frac{\mathcal{S}_{j^*}(k)W}{s^{kt}} & \leq \frac{\mathcal{S}_{j^*}(i)W}{s^{it}}  + \sum^{t-1}_{k=i+1} \frac{W}{s^{kt-1}} \\ 
& \leq  \frac{\mathcal{S}_{j^*}(i)W}{s^{it}}  +  \frac{2W}{s^{(i+1)t -1}} \\ 
& < \frac{\mathcal{S}_{j^*}(i)W}{s^{it}} + \frac{W}{s^{it}} \\
& = \frac{ (\mathcal{S}_{j^*}(i) + 1) W}{s^{it}}
\end{split}
\end{equation*}
Therefore, if Player $P_i$ inserts an interval of length $\frac{jW}{s^{it}}$ such that $j \geq \mathcal{S}_{j^*}(i) + 1$, the length is larger than the above gap and all intervals must intersect.  Since the referee has deleted all intervals with non-zero bits corresponding to indices $j$ for all $j < S_{j^*}(i)$, we are only left to consider $j \geq S_{j^*}(i)$. 

Let us first consider the case for which $X_{\mathcal{S}_{j^*}}$ is all $0$s. 
If there is a non-zero interval along any path $\mathcal{S}_{j'}$ for $j' > 
j^*$ for player $i'$, then by the analysis in the above paragraph, the right 
endpoint of such an interval covers all possible intervals inserted from the 
set $X_{\mathcal{S}_{>j'}}$. This is because the path $\mathcal{S}_{j'}$ is 
lexicographically larger than the path $\mathcal{S}_{j^*}$ and for player 
$P_i$, this corresponds to bits in the vector below the index 
$\mathcal{S}_{j^*}$, implying the index they considered while inserting the 
intervals was strictly larger $\mathcal{S}_{j^*}$. We note this is a subtle 
point, since from the player's perspective the intervals were inserting with 
length proportional to the lexicographic ordering of the paths restricted to 
index $i$. Therefore, $\alpha \leq 1$. 

Now, we consider the input where $X_{\mathcal{S}_{j^*}}$ has exactly one $1$. 
We note that this additionally contributes at most one more disjoint interval 
to the set obtained from the previous analysis. Therefore, for the first case, 
$\alpha \leq 2$.

Finally, we consider the case where $X_{\mathcal{S}_{j^*}}$ is the all $1$s 
vector. The first player inserts the interval $\left(0, \frac{\mathcal{S}_{j^*}(1) W}{s^t} \right)$, the second player inserts $\left(  \frac{\mathcal{S}_{j^*}(1) W}{s}, \frac{\mathcal{S}_{j^*}(1) W}{s^t} + \frac{\mathcal{S}_{j^*}(2) W}{s^{2t}} \right)$, and so on until the last 
player inserts $\left(  \sum^{t-1}_{k=1} \frac{\mathcal{S}_{j^*}(k)W}{s^{kt}} ,  \sum^{t}_{k=1} \frac{\mathcal{S}_{j^*}(k)W}{s^{kt}}\right)$. We observe 
that this is a set of $t$ disjoint intervals and thus $\alpha \geq t$. 
Therefore, any $(t/2)$-approximation to $\alpha$ can distinguish between the 
two cases. 
\end{proof}

Next, we prove a lower bound on the randomized communication complexity of 
\texttt{APD$_{s,t}$}. We assume familiarity with standard information theory 
terminology. We refer the reader to \cite{Bar02} for further background. Given 
the connection between simultaneous communication and streaming algorithms 
established in Theorem \ref{thm:sketch_strict_turnstile}, we can focus on 
lower bounding the randomized communication complexity of 
\texttt{APD$_{s,t}$}, denoted by 
$R_{\delta}\left(\text{\texttt{APD$_{s,t}$}}\right)$. In order to prove a 
communication lower bound, we need the following inequalities:

\begin{theorem}(\textsf{Fano's Inequality.})
Let $X$ and $Y$ be two random variables defined over the ranges $R_X$ and 
$R_Y$. Let $g:R_Y \to R_X$ be a predictor function that observes a value for 
$Y$ and guesses the corresponding value for $X$. Let $\delta$ be the error 
probability over $X,Y$, defined as $Pr\left(g(Y) \neq X\right)$. Then, 
$H_2\left(\delta\right) + \delta \log(|R_X|-1) \geq H\left(X|Y\right)$.
\end{theorem}

\begin{lemma}(\textsf{Chain Rule and Data Processing Inequality.})
Let $X$ and $Y$ be two random variables defined over ranges $R_X$ and $R_Y$. 
Let $h: R_X \to \mathcal{R}$ be a function. 
\begin{enumerate}
    \item Chain Rule for Mutual Information: $I\left(X, Y ; Z\right) = 
    I\left(X;Z\right) + I\left(X;Y | Z\right)$.
    \item Data Processing Inequality: $I\left(h(X) ; Y\right) \leq I\left(X ; Y\right)$.
\end{enumerate}
\end{lemma}

Our lower bound builds on and extends information complexity arguments in 
\cite{BJKS02}. We define a distribution $\mu$ on the input $X^1_\mathcal{S}, 
X^2_\mathcal{S}, \ldots X^t_\mathcal{S}$ as the following random process. Let 
$\left(D_1, D_2, \ldots D_{t}, \mathcal{S}_{j^*}\right)$ be a uniformly chosen 
partition of $\mathcal{S} =\{ \mathcal{S}_1, \mathcal{S}_2, \ldots 
\mathcal{S}_s \}$ such that $D_j$ represents a set of $s/t$ paths in 
$\mathcal{S}$. 
Choose the non-zero entries of $X^i_{S}$ to be indexed by a subset of $D_i(i) 
\cup S_{j^*}(i)$, where $D_i(i)$ is the $i^{th}$ entry of each path in $D_i$, 
as follows: with equal probability, either all the bits indexed by path 
$S_{j^*}$ are set to $1$ or they are all set to $0$. 
In other words, with probability $1/2$, $X_{\mathcal{S}_{j^*}}$ is set to be 
the all $1$s vector, otherwise, it is set to be the all $0$s vector. 
Then, for each path $\mathcal{S}_{j'} \in D_i$, set $X^i_{\mathcal{S}_{j'}
(j')}$ to be $\{ 0, 1\}$ uniformly and set $X^{k}_{\mathcal{S}_{j'}(j')}$ for 
$k \neq i$ to be $0$. Note, this ensures that each path $\mathcal{S}_{j'}$ has 
at most one non-zero entry. 


Further, in our communication problem, each player receives an additional 
input, which represents the normalized sum of the relevant indices of the 
previous player, i.e.,  the $i^{th}$ player receives $\ell_i = \sum^{i-1}_{k=1} \frac{\mathcal{S}_{j^*}(k)W}{s^{kt}}$. We note that our lower bound 
only holds if this additional input $\ell_i$ is uncorrelated with the answer, 
$\mathcal{S}_{j^*}(i)$. In fact, recall if $\ell_i$ were $\mathcal{S}_{j^*}
(i)$, there is an efficient protocol to solve our problem as each player would 
know what bit to send to the referee. 

\begin{theorem}(\textsf{Randomized communication complexity of } \texttt{APD$_{s,t}$}.)
\label{thm:communication_complexity_path_disj}
For all $\delta >0$, $R_{\delta}\left(\text{\texttt{APD$_{s,t}$}}\right) \geq \frac{s}{C't}\left(1 - H_2(\delta)\right)$, where $H_2$ is the binary entropy function and $C'$ is a fixed constant. 
\end{theorem}
\begin{proof}
Let $X^i_\mathcal{S}$ denote the input of the $i^{th}$ player distributed 
according to $\mu$. Let $\Pi$ denote a random variable for a $\delta$-error 
simultaneous protocol for \texttt{APD$_{s,t}$} and $\Pi_i$ denote the message 
sent by player $P_i$ to the referee. Then, the length of the message sent by 
player $P_i$ is lower bounded by the entropy of $\Pi_i$, denoted by 
$H(\Pi_i)$. Therefore, it suffices to lower bound $\sum_i H\left(\Pi_i\right) 
\geq \frac{s}{C't}\left(1 - H_2(\delta)\right)$, for a fixed constant $C'$. 
Let $F$ be the output of \texttt{APD$_{s,t}$} on $X^1_\mathcal{S}, 
X^2_\mathcal{S} \ldots X^t_\mathcal{S}$ and $D = \left(D_1, D_2, \ldots 
D_{t}\right)$ be a partition of the paths. Recall the referee's input is the 
path $\mathcal{S}_{j^*}$ and the bit vectors $X_{\mathcal{S}_{<j^*}}$, and $R$ 
is a public random string. Using Fano's inequality and the chain rule for 
mutual information, 
\begin{equation}
\label{eqn:fano_chainrule}
\begin{split}
H_2\left(\delta\right) \geq H\left(F| \Pi, R\right) & \geq H\left(F | \Pi, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) \\
& \geq H\left(F | D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) - I\left(F; \Pi | D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) \\
& = H\left(F | D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) - \sum_{i\in [t]} I\left(F; \Pi_i| \Pi_{<i}, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right)
\end{split}
\end{equation}
We then upper bound each term in the summation above. For a fixed $i \in [t]$, 
\begin{equation}
\label{eqn:upper_bound}
\begin{split}
& I\left(F; \Pi_i| \Pi_{<i}, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) \\ 
& = H\left(\Pi_i| \Pi_{<i}, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) 
- H\left(\Pi_i| F, \Pi_{<i}, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) \\
& \leq H\left(\Pi_i| D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) - H\left(\Pi_i| F, \Pi_{<i}, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right)
\end{split}
\end{equation}

The last inequality follows from the fact that conditioning does not increase 
entropy. We observe that given $F$, $D$, $\mathcal{S}_{j^*}$ and 
$X_{\mathcal{S}_{<j^*}}$, the $X^i_\mathcal{S}$'s are mutually independent 
random variables. To see this, note that the bits in 
$X^i_{<\mathcal{S}_{j^*}}$ are fixed given the conditioning. If the bits are 
indexed by $D_i(i)$ (the set of indices that correspond to the $i^{th}$ 
coordinate of all paths $S_{i'} \in D_i$) and do not correspond to an index 
that gets fixed by $X^i_{<\mathcal{S}_{j^*}}$, they are set uniformly and 
independently. Therefore, $I\left(X^i_\mathcal{S}; X^{<i}_\mathcal{S}| F, \Pi, 
D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) = 0$. Apart from the 
bit vector, $X^i_\mathcal{S}$, the $i^{th}$ player also receives $\ell_i = 
\sum^{i-1}_{k=1} \frac{\mathcal{S}_{j^*}(k)W}{s^{kt}}$, a normalized sum of 
the indices for the previous players, along path $\mathcal{S}_{j^*}$. 
Conditioning on the path $\mathcal{S}_{j^*}$ fixes the $\ell_i$s. Therefore, 
the message sent by player $P_i$ is conditionally independent of the messages 
sent by the previous players.  By the data processing inequality, 
\begin{equation}
\label{eqn:mutual_info_zero}
I\left(\Pi_i ; \Pi_{<i} | F,  D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) =0
\end{equation} 
 
Note, here we crucially use the fact that the communication model is 
simultaneous as opposed to one-way communication between the players $P_i$ and 
$P_{i-1}$ (in this case, the message sent by player $P_i$ depends on the 
messages received by the previous players and the mutual information is non-
zero). Thus, equation \ref{eqn:mutual_info_zero} implies
\begin{equation}
\label{eqn:dp_inequality}
\begin{split}
H\left(\Pi_i| F, \Pi_{<i}, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) = H\left(\Pi_i| F, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right)
\end{split}
\end{equation}
Substituting Equation \ref{eqn:dp_inequality} back in Equation \ref{eqn:upper_bound}, we get 
\begin{equation}
\label{eqn:entropy_bound}
\begin{split}
I\left(F; \Pi_i| \Pi_{<i}, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) & \leq 
H\left(\Pi_i| D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) - H\left(\Pi_i| F, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) \\
& = I\left(F ; \Pi_i | D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) \\
& = H\left(F|D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) - H\left(F | \Pi_i, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right)
\end{split}
\end{equation}
Observe, $H\left(F|D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) = 1$, since conditioned on $D, \mathcal{S}_{j^*}$ and  $X_{\mathcal{S}_{<j^*}}$, 
$F$ is defined to be uniform on $\{0, 1\}$. Now consider the conditioning of 
the second term above. Since $D_i$ is fixed given $D^{-i}= \bigcup_{\forall i' 
\neq i} D_{i'}$, and $S_{ j^*}$, we have $H\left(F | \Pi_i, D, 
\mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right) =  H\left(F | \Pi_i, D^{-
i}, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right)$. Let $E$ be the event 
that $D^{-i}=d$ and $X_{\mathcal{S}_{<j^*}}=x$. Then,
\begin{equation}
\label{eqn:expanding_entropy}
\begin{split}
H\left(F | \Pi_i,D,\mathcal{S}_{j^*},X_{\mathcal{S}_{<j^*}},R\right) & = H\left(F | \Pi_i,D^{-i},\mathcal{S}_{j^*},X_{\mathcal{S}_{<j^*}},R\right) \\
& = \sum_{d,x} \Pr(E) H\left(F | \Pi_i, \mathcal{S}_{j^*}, E, R\right)
\end{split}
\end{equation}


Let $\sigma_i$ be the complement of the union of the sets in $d$. Note, $\sigma_i$ corresponds to the subset of indices of the input to player $P_i$ that are assigned to him according to $D_i$ and thus is a set of size $\frac{s}{t}$. Conditioning on the fixing $x$, along the $j-1$ paths lexicographically less than $\mathcal{S}_{j^*}$ fixes a subset of the indices in $\sigma_i$. Let this set be denoted by $\sigma_{i|x}$. Next, we show that $|\sigma_{i|x}| \geq \frac{s}{ct}$, for some constant $c$, with probability at least $1 - \frac{1}{c}$. Recall, $\mathcal{S}_{j^*}(i)$ is uniform over $[s]$, therefore with probability at least $1-1/c'$, $s/c'$ indices are not fixed given $E$. Note, the set $\sigma_i$ is chosen uniformly from $[s]$. Let $W_{k}$ be an indicator random variable for the $k^{th}$ index of $\sigma_i$ being not fixed, conditioned on $s/c'$ indices not being fixed given event $E$. Let $W = \sum_{k} W_k$. Then, $\expec{}{W} = \frac{s}{c's}\cdot \frac{s}{t} = \frac{s}{c't}$.  By a Chernoff bound, 
\[
\Pr \left[ W \leq (1-\delta)\expec{}{W} \right] \leq \textrm{exp}\left(-\frac{\delta^2 \expec{}{W}}{2}\right) = \textrm{exp}\left(-\frac{\delta^2 s}{2c't}\right) 
\]
Therefore, setting $\delta = 1/2$, with probability at least $1 - \textrm{exp}\left(-\frac{ s}{8c't}\right)$,  $W \geq \frac{s}{2c't}$. Union bounding over the two events, and observing $W$ is exactly $|\sigma_{i|x}|$, with probability at least $1 - 1/c$, $|\sigma_{i|x}|\geq \frac{s}{ct}$, for any constant $c$. 

Thus, $X^i_S$, the input for the $i^{th}$ player, has non-zero non-fixed entries in indices that are a subset of $\sigma_{i|x}$, given $E$. 
%By Lemma, we know that $|\sigma_{i|x}| \geq \frac{s}{ct}$, for some constant $c$, with high probability. 
Let $Z_l$ for $l \in \sigma_{i|x}$ be an indicator random variable for the $l^{th}$ bit of $X^i_S$ being set to $1$. Given $E$, the $Z_l$'s completely determine the $X^i_S$'s and vice-versa. Moreover, given $E$ and $S_{ j^*}(i) = l$, $F = Z_l$.  Therefore, substituting this in Equation \ref{eqn:expanding_entropy}, we get 
\begin{equation}
\label{eqn:entropy_sigma}
\begin{split}
H\left(F | \Pi_i, \mathcal{S}_{j^*}, E, R\right) & = \sum_{l\in \sigma_{i|x}} \Pr\left(\mathcal{S}_{j^*}(i)=l | E, R\right) H\left(F | \Pi_i, \mathcal{S}_{j^*}(i)=l, E, R\right) \\
& = \sum_{l \in \sigma_{i|x}} \frac{H\left(Z_l | \Pi_i, \mathcal{S}_{j^*}(i)=l, E, R\right)}{|\sigma_{i|x}|}
\end{split}
\end{equation}

Now, by Lemma \ref{lem:conditional_ind}, we know that given $E$, $X^i_S$ and $\mathcal{S}_{j^*}(i)$ are independent. Therefore, $Z_l$ is independent of $\mathcal{S}_{j^*}(i)$ given $E$. Now, $\Pi_i$ is a function of $X^i_S$ and $\ell_i = \sum^{i-1}_{k=1} \frac{\mathcal{S}_{j^*}(k)}{s^{kt}}$. 
Since $\ell_i$ is a normalized sum of uniformly random indices and independent of $\mathcal{S}_{j^*}(i)$, $\Pi_i$ is independent of $\mathcal{S}_{j^*}(i)$ given $E$. Crucially this does not hold if the integer given to the $i^{th}$ player is $\mathcal{S}_{j^*}(i)$. It follows that $H\left(Z_i | \Pi_i, \mathcal{S}_{j^*}(i)=l, E, R\right) = H\left(Z_i | \Pi_i, E, R\right)$. Therefore, 
\begin{equation}
\begin{split}
H\left(F | \Pi_i, \mathcal{S}_{j^*}, E, R\right) & = \sum_{l \in \sigma_{i|x}} \frac{H\left(Z_l | \Pi_i, E, R\right)}{|\sigma_{i|x}|} \\
& \geq \frac{H\left(Z_1, Z_2 \ldots Z_{|\sigma_{i|x}|} | \Pi_i,  E, R\right)}{|\sigma_{i|x}|} \\
& =\frac{H\left(X^i_S| \Pi_i, E, R\right)}{|\sigma_{i|x}|}
\end{split}
\end{equation}
where the inequality follows from the sub-additivity of the entropy function. Substituting this bound into Equation \ref{eqn:expanding_entropy}, we get 
\begin{equation}
\begin{split}
H\left(F | \Pi_i,D,\mathcal{S}_{j^*},X_{\mathcal{S}_{<j^*}},R\right) & \geq \frac{H\left(X^i_S| \Pi_i,  E, R\right)}{|\sigma_{i|x}|} \\
& \geq \frac{H\left(X_S^i| \Pi_i, D, X_{\mathcal{S}_{<j^*}},R\right)}{|\sigma_{i|x}|} \\
& \geq \frac{H\left(X_S^i| D,  X_{\mathcal{S}_{<j^*}}, R\right) - H\left(\Pi_i| D, X_{\mathcal{S}_{<j^*}}, R\right)}{|\sigma_{i|x}|}
\end{split}
\end{equation}


Observe, $H\left(X^i_S| D,  X_{\mathcal{S}_{<j^*}}, R\right)$ is non-zero for the bits not fixed by the conditioning. Since $\mathcal{S}_{j^*}$ is chosen uniformly at random, in expectation, a constant fraction of $X^i_S$ is not fixed by the conditioning. Therefore, $H\left(X^i_S| D,  X_{\mathcal{S}_{<j^*}}, R\right) \geq \frac{|\sigma_{i|x}|}{C}$, for a fixed constant $C$. The second term simplifies to $\frac{H(\Pi_i)}{|\sigma_{i|x}|}$. Plugging this back into the above, we get
$H\left(F | \Pi_i, D, \mathcal{S}_{j^*}, X_{\mathcal{S}_{<j^*}}, R\right)  \geq \frac{c\cdot C}{s/t} - \frac{c\cdot H\left(\Pi_i\right)}{s/t}$.
Combining this with Equations \ref{eqn:fano_chainrule} and \ref{eqn:entropy_bound} we finish the proof of the theorem.  
\end{proof}

\begin{lemma}
\label{lem:conditional_ind}
Let $X^i_{\mathcal{S}}$ be the input for player $P_i$ and let $\mathcal{S}_{j^*}$ be the path given to the referee. Let $D = (D_1, D_2, \ldots, D_t)$ be a partition of the set of paths $\mathcal{S}$, such that for all $i\in[t]$, $D_i$ has $s/t$ paths. Let $E$ be the event that $D^{-i}=d$ and $X_{\mathcal{S}_{<j^*}}=x$. Then, conditioned on event $E$, $X^{i}_{\mathcal{S}}$ and $\mathcal{S}_{j^*}$ are independent. 
\end{lemma}

Next, we formalize the connection between the randomized communication 
complexity of a problem in the simultaneous communication model and the space 
complexity of one-pass turnstile streaming algorithms. Here, we use the 
characterization of strict turnstile streams as linear sketches and use a 
corollary from Weinstein and Woodruff \cite{DBLP:conf/icalp/WeinsteinW15}. 
Note, their corollary, as written is not true for strict turnstile streams, 
since they use results of \cite{DBLP:conf/stoc/LiNW14}. However, this can be 
fixed by simply combining it with Theorem \ref{thm:sketch_strict_turnstile}.  
 
\begin{lemma}(Combining Corollary 5.7 in \cite{DBLP:conf/icalp/WeinsteinW15} and Theorem \ref{thm:sketch_strict_turnstile}.)
\label{lem:bride_streaming_communication}
Let $R_{\delta}\left(\text{\texttt{APD$_{s,t}$}}\right) = \eta$. Let \texttt{Alg} be a space-optimal streaming algorithm in the strict turnstile 
model such that \texttt{Alg} can be used to solve \texttt{APD$_{s,t}$} with 
probability at least $1-\delta$. Then, the space complexity of \texttt{Alg} is 
at least $\eta/t$. 
\end{lemma} 


\textbf{Proof of Theorem \ref{thm:lowerbound_arb_len_unit_wt_ins_del}.}
By Theorem \ref{thm:communication_complexity_path_disj}, we know that the 
randomized communication complexity of \texttt{APD$_{s,t}$}, denoted by $R_{\delta}\left(\text{\texttt{APD$_{s,t}$}}\right)$, is  $\Omega\left(\frac{s\log(s/t)}{t}\right)$. Observe, a lower bound on the 
randomized communication complexity implies a lower bound on the size of the 
linear sketch, which is at most the space complexity of the streaming 
algorithm. Therefore, Lemma \ref{lem:bride_streaming_communication} implies 
that the space complexity of \texttt{Alg} is at least 
$\Omega\left(\frac{s\log(s/t)}{t^2}\right)$ bits. Setting $t = 2c$ and $s = n/t$, the space complexity of \texttt{Alg} is at least $\Omega(n)$ words and 
Theorem \ref{thm:lowerbound_arb_len_unit_wt_ins_del} then follows from Lemma \ref{lem:streamingreduction}. 
